DesignCoder: Hierarchy-Aware and Self-Correcting UI Code Generation with Large Language Models

Multimodal large language models (MLLMs) have streamlined front-end interface development by automating code generation. However, these models also introduce challenges in ensuring code quality. Existing approaches struggle to maintain both visual consistency and functional completeness in the generated components. Moreover, they lack mechanisms to assess the fidelity and correctness of the rendered pages. To address these issues, we propose DesignCoder, a novel hierarchical-aware and self-correcting automated code generation framework. Specifically, we introduce UI Grouping Chains, which enhance MLLMs' capability to understand and predict complex nested UI hierarchies. Subsequently, DesignCoder employs a hierarchical divide-and-conquer approach to generate front-end code. Finally, we incorporate a self-correction mechanism to improve the model's ability to identify and rectify errors in the generated code. Extensive evaluations on a dataset of UI mockups collected from both open-source communities and industry projects demonstrate that DesignCoder outperforms state-of-the-art baselines in React Native, a widely adopted UI framework. Our method achieves a 37.63%, 9.52%, 12.82% performance increase in visual similarity metrics (MSE, CLIP, SSIM) and significantly improves code structure similarity in terms of TreeBLEU, Container Match, and Tree Edit Distance by 30.19%, 29.31%, 24.67%. Furthermore, we conducted a user study with professional developers to assess the quality and practicality of the generated code. Results indicate that DesignCoder aligns with industry best practices, demonstrating high usability, readability, and maintainability. Our approach provides an efficient and practical solution for agile front-end development, enabling development teams to focus more on core functionality and product innovation.

==> sections/method.tex <==
\section{Approach}
% However, design metadata is often lengthy, requiring processing a large amount of irrelevant input, which not only reduces performance but may also lead to code generation failures. To address this issue, 
Figure \ref{fig:overview} illustrates the overall workflow of our method, DesignCoder, which takes UI design mockups as input. DesignCoder aims to accelerate development and iteration in real-world industrial scenarios, where visual consistency, code maintainability, and usability are critical. By leveraging design metadata, our method can acquire design information to enhance the quality of generated code. DesignCoder introduces the UI Grouping Chain (Section 3.1), which consists of two key steps: (1) Visual Processing: This step segments UI screenshots into subregions based on visual semantics. (2) Grouping Reasoning: MLLM employs a two-stage prompting strategy to analyze the semantics of elements within each subregion. It then integrates these semantics with visual prompts to guide the MLLM in constructing some hierarchical UI component sub-tree. In the code generation step (Section 3.2), we adopt a divide-and-conquer strategy, where each sub-tree is processed independently. The design metadata are used to generate CSS styles, and the layout and styles are integrated into a unified prompt to guide MLLM in generating code. Finally, in the self-correcting code refinement step (Section 3.3), our method iteratively verifies and corrects the initial generated code through visual comparison to ensure visual consistency and correctness.

\begin{figure*}[thp]
\centering
\includegraphics[width=0.9\textwidth]{figures/method.pdf}
\vspace{-0.1in}
\caption{The overview of DesignCoder.}
\label{fig:overview}
\vspace{-0.05in}
\end{figure*}

\subsection{UI Grouping Chain}
% 先讲下问题的背景，在引出用什么方法来解决

% 详细讲述方法，配上标准化的公式（先给出公式，where xx给出解释）

% 当上一步完成后，利用生成的布局树进行代码生成。

% 使用MLLM直接根据UI图像生成组件树是很困难的，因为涉及到确定组件的bbox。MLLM通常在处理简单任务时表现出令人满意的性能，这在UI领域同样适用。为了简化任务复杂度，我们提出了UI Grouping Chain，用来progressively生成组件树。具体而言，我们提出了a visual processing prompt that segments the UI image into sub-images。xx使用separation line detector来分割web页面，然而移动端页面通常不具备明显 separation line。因此，我们首先提取metadata中的layer id、bbox和type（比如，shape、text），to form a layer list。然后，输入图像I和layer list，我们使用visual processing prompt来将layer list分为多个sub list。我们根据sub list中的layer bboxes的并集来算出sub-image的bbox。该过程可表示如下：
\begin{figure}[thp]
\centering
\includegraphics[width=0.48\textwidth]{figures/prompt.pdf}
\vspace{-0.15in}
\caption{The prompt used to construct UI grouping chain.}
\vspace{-0.1in}
\label{fig:prompt}
\end{figure}

Directly generating a component tree from a UI image using MLLM is very challenging because it involves determining the components’ bounding boxes. MLLM typically exhibits satisfactory performance on simple tasks, which also applies in the UI domain. To simplify the task complexity, we propose the UI Grouping Chain, which is used to progressively generate the component tree. Specifically, we introduce a visual processing prompt that segments the UI image into sub-images. Some approaches use a separation line detector to segment web pages; however, mobile pages typically do not have distinct separation lines. 

Therefore, we first extract the layer \(id\),  \({bbox}\), and \(\text{type}\) (e.g., shape, text) from the metadata to form a layer list \(L_{\text{layers}}\). Then, given the input image \(I\) and the \(L_{\text{layers}}\), we use the visual processing prompt \(P\_{visual}\) to divide \(L_{\text{layers}}\) into multiple sublists \(L_{\text{sub\_layers}}\). We compute the bounding box of each sub-image based on the union of the layer bounding boxes in each sublist. This process can be expressed as follows:
\begin{equation}
    L_{\text{layer}} = \big\{ (id_k, \mathbf{bbox}_k, \text{type}_k) \big\}_{k=1}^{N}
\end{equation}
\begin{equation}
    L_{\text{sub\_layers}} = P_\text{visual}(I, L_{\text{layers}})
\end{equation}
% 我们观察到仅根据layer的bbox得到的成组关系存在组件遗漏，通过规则成组容易出错。因此，我们借助图层之间的语义关系，将语义近似的图层成组为组件。我们应用一个语义分析prompt P\_semantic来生成layer sub-list中的layer语义。比如，对于一个search bar中的文本，生成的语义描述为：“A placeholder text displaying 'Search for fruit salad combos,' which suggests the intended search scope or example use case for the search bar.” 最终，我们得到layer语义list L\_semantic。随后，我们应用一个prompt P\_grzoup来生成子组件树。由于我们的子组件树按顺序存储，因此可以简单地重建为完整的组件树。组件树中的非叶子节点就是一个组件，并以其功能命名，比如：“merged\_SearchSection”、“merged\_CategoryTabs”。
% 最终，Grouping results 包含了子组件树提供了完整的组件功能性描述以及层级结构，子图提供了视觉参考，从而帮助MLLM understand complex design intent and reduce the difficulty of code generation.
We observed that grouping relationships derived solely from layer bboxes often result in missing components, and rule-based grouping is prone to errors. To address this issue, we leverage semantic relationships between layers, grouping semantically similar layers into components. Specifically, we apply a semantic analysis prompt, \(P\_semantic\), to generate semantic descriptions for layers in the layer sub-list. For example, for text within a search bar, the generated description might be: \textit{"A placeholder text displaying 'Search for fruit salad combos,' which suggests the intended search scope or example use case for the search bar."} This process yields a layer semantic list \(L\_semantic\). We then use a grouping prompt \(P\_group\) to generate a sub-component tree, which is stored sequentially and can be easily reconstructed into a complete component tree. In this structure, non-leaf nodes represent functional components and are named accordingly, such as \textit{"merged\_SearchSection"} or \textit{"merged\_CategoryTabs"}. This process can be expressed as follows:
\begin{equation}
    L_{\text{semantic}} = P_{\text{semantic}}(L_{\text{sub\_layers}}, I_{\text{sub}})
\end{equation}
\begin{equation}
    L_{\text{sub\_tree}} = P_{\text{group}}(L_{\text{semantic}}, I_{\text{sub}})
\end{equation}

The grouping results include the sub-component tree, which provides a structured functional description of the complete component hierarchy, while the sub-images serve as visual references, helping MLLMs understand complex design intent and reducing the difficulty of code generation.

\subsection{Hierarchy-Aware Code Generation}
% 先讲下问题的背景，在引出用什么方法来解决

% 详细讲述方法，配上标准化的公式（先给出公式，where xx给出解释）

% 当上一步完成后，利用生成的布局树进行代码生成。
% 最后，在本节中，我们将介绍生成 UI 前端代码的方法，该方法主要分为两部分：HTML 架构和 CSS 样式代码。借鉴这些见解，我们决定将布局生成（HTML）和样式生成（CSS）的任务分开（图 1 d）。这种方法利用了 LLM 在文本生成方面的优势来生成 CSS 代码，同时保持 UI 布局树对 HTML 代码结构的强大引导作用。我们首先展示如何从 UI 布局树中推导出 HTML 代码。对于任何非叶节点，我们用 <div> 标签将其封装起来，并遍历以它为根的子树，使用 <div> 标签的嵌套结构来描绘整个骨架布局。对于代表图像和文本的叶节点元素，我们分别应用 <img> 和 <span> 标签。利用 UI 元素类别识别的结果，我们为每个元素分配一个类名作为 CSS 选择器。CSS 样式决定了页面上元素的呈现效果。CSS 样式有两种类型：布局相关的属性决定了元素在页面上的呈现位置；视觉效果相关的属性则确保 UI 的美观性。先前的研究 [9, 32] 主要支持绝对尺寸布局，导致页面无法响应设备尺寸，这不利于进一步的开发和维护。考虑到这一点，我们采用一种可以响应设备尺寸的弹性布局模型。对于每个被 <div> 包裹的元素，我们根据第 3.2 节中设置的属性确定布局方法。对于具有“need_absolute”属性的节点，我们将它们的 CSS “position” 属性设置为“relative”，并将它们的子元素的“position”属性设置为“absolute”。在此，子节点是基于父节点的左上角坐标进行绝对定位，设置它们的“top”和“left”属性。如果一个子节点符合行或列排列的特征，我们就将父节点的“position”属性设置为“flex”，并根据第 3.2 节中确定的“flex-direction”属性将其排列成行或列。每个子节点的“margin-top”和“margin-left”属性由它们与父节点或相邻节点的距离决定。“width”和“height”属性可以根据设计原型中的参数直接获取。最后，我们描述如何利用诸如 GPT-4 [33] 这样的大型语言模型来生成其余与视觉效果相关的 CSS 属性。我们的提示包括四个部分：<角色扮演、用户输入、字段解释、输出要求>。在角色扮演部分，我们以一位有多年经验且技术精湛的前端开发者的身份提示大型语言模型。对于用户输入，基于 Figma API 用户文档 [34]，我们过滤掉与视觉效果无关的样式信息，并将剩余的信息以字典键值对的形式整理出来。在字段解释部分，我们再次回顾了 Figma API 文档，并将所有相关样式属性的解释性文本存储为一个 JSON 文件，以便让语言模型理解设计原型中的样式。在输出要求中，我们指示语言模型返回一个可解析的 JSON，其中每个字段对应一个相关的 CSS 属性及其值。

% 如何确保生成的代码完全遵循生成的组件树
Although the generated UI layout tree captures certain component semantics and hierarchical structures, two key aspects remain missing: (1) Style code for leaf nodes. To generate an interface that visually aligns with the input UI design, accurately understanding style information is crucial. Design Metadata can assist MLLM in interpreting design semantics, but some metadata may be excessively verbose and contain irrelevant information, requiring further filtering and processing. (2) Attributes and styles of container nodes in the layout tree. To enhance the quality of code generated by MLLM, we designed a layout-tree-based generation process.

Specifically, we introduce Prompt \(P\_style\), where the style information of leaf nodes is separately fed into MLLM to predict the corresponding CSS code (as shown in the figure). The generated CSS code is then embedded into the corresponding sub-layout tree, forming an intermediate representation that includes style information. Next, we construct Prompt \(P\_code\), which takes the intermediate representation and its corresponding sub-image as input to MLLM for analyzing the global layout and functional attributes, further refining the styling information of container nodes (e.g., color, margins, paddings, and other CSS properties) and assigning appropriate component tags (such as <Button>, <ScrollView>, and <List>). For instance, in the case of a button component, if MLLM generates a <div> instead of a <Button> purely based on the DOM structure, the hierarchical relationship might be correct, but the semantic accuracy of the code would still be compromised. Our approach correctly identifies the interactive nature of the component, ensuring that the generated code selects <Button> rather than a generic <div>. Similarly, for scrollable views, if the design explicitly specifies a scrolling behavior, our model can automatically choose the <ScrollView> component instead of merely applying overflow: scroll, improving both code readability and component consistency.

\subsection{Self-correcting Code Refinement}

The code generated by MLLMs may contain various errors, including missing elements, style distortions, layout inconsistencies, syntax errors, and functional anomalies. While existing studies \cite{zhou2024bridging, jiang2024rocode} focus on ensuring correct code parsing and execution, correct parsing does not necessarily guarantee that the generated code is visually and functionally accurate. For instance, the generated code may omit the search icon within the search bar or result in a disorganized element layout, ultimately affecting usability. To address these issues, we propose a self-correcting strategy based on the generated component tree, which systematically evaluates the visual consistency and responsive layout of the generated code. We then employ a divide-and-conquer approach to perform fine-grained code corrections and merge the refined code.

Specifically, we leverage Appium—a UI automation testing tool—to capture rendered page screenshots and extract component attributes, including bounding boxes, element types, text content, and hierarchical structures. Next, we match the rendered components using node IDs from the component tree. Then, we extract image segments based on each component’s bounding box, obtaining the original component image \( I_j \) and the rendered component image \( I_k \).

We then employ a visual analysis prompt, \( P_{\text{analysis}} \), to meticulously compare these images, focusing on identifying any element misarrangement or style errors in the generated code:
\begin{equation}
S_i = P_{\text{analysis}}(I_j, I_k)   
\end{equation}

where \( S_i \) represents the repair suggestion for the \( i \)-th component, with \( I_j \) corresponding to the original image and \( I_k \) to the rendered image.

Subsequently, the generated repair suggestion \( S_i \) is combined with the associated component code snippet to form a structured code repair prompt \( P_{\text{repair}} \):
\begin{equation}
P_{\text{repair}} = \{ \text{``component\_code\_i''},\ S_i \}
\end{equation}

This prompt guides the MLLM in performing targeted code repairs. Notably, since each component can be repaired independently, the process can be parallelized, greatly enhancing the efficiency of code repair. Finally, we merge the code snippets according to the component tree order to produce the final rendered page.


\begin{figure}[thp]
\centering
\includegraphics[width=0.46\textwidth]{figures/FixedCode.pdf}
\vspace{-0.1in}
\caption{Examples of the rendering results from both the initially generated code and the refinement code. The red boxes highlight misaligned elements, the blue boxes indicate visual distortions, and the yellow boxes mark missing elements.}
\vspace{-0.1in}
\label{fig:fix}
% \vspace{-0.1in}
\end{figure}

==> sections/motivation.tex <==
\section{Background and Motivations}

In front-end development, implementing a user interface involves translating design specifications from mockups into functional code. Developers rely on these mockups to implement styles accurately, ensuring consistency in attributes such as size, color, typography, and hierarchical structure. Such design information is essential for generating high-fidelity UI code and achieving precise final rendering. However, manually translating mockups into code remains a time-consuming process, requiring developers to meticulously implement styles and layout structures. Recent advancements in AI-assisted automation provide new opportunities to streamline this process.
% MLLM在使用Screenshot成代码的过程中还是存在问题，问题包括两个：视觉不一致；组件代码不完整
However, despite the potential of MLLMs in UI code generation, current MLLMs still face significant challenges when processing UI design mockups. As illustrated in Figure 1, we take a Figma design as an example and provide the UI screenshot to an MLLM (GPT-4o) to illustrate some of the issues encountered in generating UI code. We did not provide design metadata, as it typically consists of thousands of lines of JSON data, which would instead degrade the performance of MLLMs.

\textbf{Element Misarrangement.} Even when provided with design metadata that includes a hierarchical structure, MLLMs fail to correctly position or order elements relative to their adjacent components or the overall design layout. As shown in Figure 1a, while the two product cards are correctly arranged in parallel, the "Add" button within each card is mistakenly placed in the next row. This indicates that the MLLM-generated code does not fully capture the hierarchical relationships within the UI, which may result in incorrect UI rendering and even impact the software's interaction experience.

\textbf{Element Omission.} Figure 1b illustrates another common issue in MLLM-generated UI code: the omission of certain original UI elements, such as the search and settings icons. Zhou et al. \cite{zhou2024bridging} attempted to address this problem by integrating an unsupervised detection model; however, we argue that detection models without task-specific training still suffer from performance limitations, particularly in complex nested element scenarios. For example, in Figure 1b, the detection model failed to identify the icon element within the search bar, resulting in missing UI components in the generated output.

\textbf{Element Distortion.} UI design metadata not only defines the hierarchical relationships between elements but also includes their style information. Since design metadata often exceeds several thousand tokens, MLLMs struggle to accurately extract information and interpret design styles. This results in elements being reproduced inaccurately in terms of shape, size, or color. Figure 1c illustrates this issue, where the background image has an incorrect size, and the gradient transition from black to white is missing.

\textbf{Component-Based Code Implementation and Reliability Issues.} To minimize manual code adjustments, developers expect the generated code to accurately identify interactive components within the UI and provide foundational interaction logic for further implementation. Moreover, as shown in Figure 1d, directly using screenshots and metadata does not fully ensure visual consistency between the design and the rendered UI. These discrepancies require significant manual intervention, ultimately offsetting the time-saving advantages of MLLMs in UI code generation.

These challenges highlight the current limitations of MLLMs in UI code generation. While the prospects of automated application development are promising, significant improvements are still needed in UI hierarchical structure understanding, code-visual consistency, and component-based code implementation. Addressing these issues is crucial for advancing code generation automation and streamlining application development.
